Does the fireball found in AuAu collisions at RHIC resemble plasma?

General properties of the hot and dense hadron matter (fireball) discovered in AuAu collisions with pSNN = 130 and 200 GeV at RHIC are compared with these for ideal electromagnetic plasma. None of them was found to be in contrary to those of the plasma typical signs distinguishing its from other aggregate states of the matter. The author notes that modern experimental data about the fireball properties are limited to make their comprehensive comparison with plasma signatures. The author also points out the directions needed to be studied to answer question whether the hadron matter observed in the RHIC experiments is a color analogue of the electromagnetic plasma or not.

==> zulkarneev_article_tables.eng.tex <==

\begin{table}
\caption{Summary of comparative features of the electron plasma and fireball produced in the collisions at RHIC and SPS, CERN.}
\begin{tabular}{ | p{1.0cm} | p{4.0cm} | p{4.0cm} | p{4.0cm} | c |} \hline
 \multicolumn{2}{| p{5.0cm} |}{\textbf{Properties - features of the electron plasma}} & \textbf{Fireball properties – analogues of the electromagnetic plasma}
 & \textbf{Experimental confirmation} & \textbf{References} \\ \hline
 1 & quasineutrality of the total electric charge & neutrality of the total color charge & is present & \cite{14} \\ \hline
 2 & charge separation the plasma volume (dissociation of atoms) & deconfinement of the quarks of nucleon & is absent & - \\ \hline
 3 & collective character of the particle interactions & collective character of quark interactions in the fireball medium & is present & \cite{15},\cite{17} \\ \hline
 4 & Presence of the quasi-particle excitations in the system & presence of quasi-particle excitations in the fireball medium & there are experimental indications
   & \cite{17},\cite{19}-\cite{21} \\ \hline
 5 & field screening of electric charges & screening of the color charge field & there are experimental indications & \cite{25}-\cite{27} \\ \hline
 \end{tabular}
 \label{tab:tb_01}
\end{table}
 
 
\begin{table}
\caption{Summary of the QGP signatures according to its definitions in [\cite{1}-\cite{9}].}
\footnotesize{
\begin{tabular}{ |c| p{4.0cm} | c |c|c|c|c|c|c|c| p{2.5cm} |} \hline
  &                                                        & 1980 & 1983 & 1984/86 & 1984 & 1989 & 1996 & 1999 & 2004 & 2005 \\ \hline
1 &  Deconfinement of quarks                               &   +  &   +  &    +    &   +  &   +  &   +  &   +  &   +  &   +  \\ \hline
2 &  Energy necessary for quark deconfinement		   &   +  &   +  &    +    &   +  &   -  &   + ($> T_{c}$)  &   +  &   +  &   -  \\ \hline
3 &  Size of plasma bigger than nucleon size               &   -  &   -  &    +    &   +  &   +  &   -  &   +  &   -  &   +  \\ \hline
4 &  Independence of quark motion                          &   -  &   +  &    +    &   +  &   +  &   -  &   -  &   -  &   thermalization of constituents \\ \hline
5 &  Chiral symmetry restoration	                   &   -  &   +  &    -    &   -  &   -  &   -  &   +  &   +  &   -  \\ \hline
6 &  Smallness of quark masses                             &   -  &   +  &    -    &   -  &   -  &   +  &   -  &   -  &   -  \\ \hline
  &  References                         & \cite{1} & \cite{2} & \cite{3} & \cite{4}  & \cite{5}  & \cite{6} & \cite{7} & \cite{8} & \cite{9} \\ \hline
\end{tabular}
}
\textbf{Note: signs ‘‘+/-’’ mean that the indicated feature is or not necessary in the given definition of plasma; 
$T_{c}$ – is a temperature of phase transition from the nucleon matter to QGP.}
\label{tab:tb_02}
\end{table}


